SVFusion: A CPU-GPU Co-Processing Architecture for Large-Scale Real-Time Vector Search

Approximate Nearest Neighbor Search (ANNS) underpins modern applications such as information retrieval and recommendation. With the rapid growth of vector data, efficient indexing for real-time vector search has become rudimentary. Existing CPU-based solutions support updates but suffer from low throughput, while GPU-accelerated systems deliver high performance but face challenges with dynamic updates and limited GPU memory, resulting in a critical performance gap for continuous, large-scale vector search requiring both accuracy and speed. In this paper, we present SVFusion, a GPU-CPU-disk collaborative framework for real-time vector search that bridges sophisticated GPU computation with online updates. SVFusion leverages a hierarchical vector index architecture that employs CPU-GPU co-processing, along with a workload-aware vector caching mechanism to maximize the efficiency of limited GPU memory. It further enhances performance through real-time coordination with CUDA multi-stream optimization and adaptive resource management, along with concurrency control that ensures data consistency under interleaved queries and updates. Empirical results demonstrate that SVFusion achieves significant improvements in query latency and throughput, exhibiting a 20.9x higher throughput on average and 1.3x to 50.7x lower latency compared to baseline methods, while maintaining high recall for large-scale datasets under various streaming workloads.

==> chapters/coverletter.tex <==
\tcbset{
    enlarge top initially by = 0.4em, 
    enlarge bottom finally by = -0.4em, 
    enlarge left by = -0.2em, 
    enlarge right by = -0.2em, 
    width = \linewidth + 0.4em, 
    colframe = gray!10, 
    sharp corners, 
    left = 0.2em, right = 0.2em, 
    top = 0em, bottom = 0em, 
    boxsep = 0em, boxrule = 0em,
    }

\newcounter{metareviewer}
\setcounter{metareviewer}{0}
\newcounter{metaweakpoint}[metareviewer]
\setcounter{metaweakpoint}{1}

\renewcommand{\themetaweakpoint}{MR.W\arabic{metaweakpoint}}
\newcommand{\themetareviewersection}{\section*{RESPONSE TO META-REVIEWER}}

\newenvironment{metareviewersection}
   {\refstepcounter{metareviewer} \themetareviewersection}
      
\newenvironment{metaweakpoint}
   {
    \refstepcounter{metaweakpoint} \noindent  
    \begin{tcolorbox}[]
    \underline{\textbf{\themetaweakpoint}}:\ \itshape
   }
   {
    \end{tcolorbox}
   }

% zl: set the reviewer number here.
\newcounter{reviewer}
\setcounter{reviewer}{0}

\newcounter{weakpoint}[reviewer]
\setcounter{weakpoint}{1}

\newcounter{detailpoint}[reviewer]
\setcounter{detailpoint}{1}

\newcounter{addiremark}[reviewer]
\setcounter{addiremark}{1}

\renewcommand{\theweakpoint}{R\arabic{reviewer}.W\arabic{weakpoint}} 
\renewcommand{\thedetailpoint}{R\arabic{reviewer}.D\arabic{detailpoint}} 
\renewcommand{\theaddiremark}{ADDITIONAL REMARKS.M\arabic{addiremark}} 

\newcommand{\thereviewersection}{\section*{RESPONSE TO REVIEWER \#\thereviewer}}

\newenvironment{reviewersection}
   {\refstepcounter{reviewer} \thereviewersection}

\newenvironment{weakpoint}
   {
    \refstepcounter{weakpoint} \noindent 
    \begin{tcolorbox}[]
    \underline{\textbf{\theweakpoint}}:\ \itshape
   }
   {
    \end{tcolorbox}
   }
   
\newenvironment{detailpoint}[1][]
   {
    % 如果提供了可选参数，使用手动编号；否则自动递增
    \ifx\relax#1\relax
        \refstepcounter{detailpoint}
    \else
        \setcounter{detailpoint}{#1}
        \refstepcounter{detailpoint}
        \addtocounter{detailpoint}{-1}
    \fi
    \noindent 
    \begin{tcolorbox}[]
    \underline{\textbf{\thedetailpoint}}:\ \itshape
   }
   {
    \end{tcolorbox}
   }

\newenvironment{addiremark}
   {\refstepcounter{addiremark} \noindent {\underline{\textbf{\theaddiremark}}:}\ \itshape}


\newenvironment{response}[1]
   {\noindent \textbf{RESPONSE}:\  }

% \onecolumn

% \centerline{\textbf{\Large Response to Reviewers' Comments}}
% \vspace{2mm}


% \begin{multicols}{2}

\newenvironment{figurecl}[1][]
  {\def\@captype{figure}\begin{center}}
  {\end{center}}

% \newenvironment{tablecl}
% {\def\@captype{table}\renewcommand{\figurename}{Table}}
% {}

\makeatletter
\def\@captype{figure}
\makeatother

\setcounter{page}{1}
% zl: end of my commands

% \noindent To PC co-chairs, meta reviewer, and reviewers:

We sincerely appreciate the reviewers and the meta-reviewer for their insightful and constructive comments.
We have carefully addressed each comment in the revised manuscript.
In this cover letter, we first summarize the major changes and then provide point-by-point responses to the concerns raised by each reviewer. 
For \zl{the} ease of reading, we have highlighted the changes in the revised paper in \changeone{blue}.

\section{Revision Summary}
We have substantially strengthened the paper in the following aspects, directly addressing the reviewers’ concerns:

\begin{enumerate}[leftmargin=*]
\item \textbf{Latency Analysis for Real-time Applications}: We have added concrete real-world \zl{use cases of} streaming ANNS in \hl{Section~\ref{sec:intro}} and redesigned the real-time coordination mechanism in \hl{Section~\ref{sec:coordination}} with CUDA multi-stream optimization and adaptive resource management. In \hl{Section~\ref{sec:sanns_performance}}, we have added comprehensive latency analysis across varying QPS rates. \zl{
(Addressing \textcolor{Purple}{\ref{mrw1}, \ref{mrw3}, \ref{r1w1}, \ref{r1d6}, \ref{r2d1}, \ref{r3d1}})
}

\item \textbf{Concurency Control}: We have reorganized \hl{Section~\ref{sec:cc_update}} to present a novel two-level concurrency control protocol to ensure data consistency across GPU-CPU-disk tiers. We have added evaluation in \hl{Section~\ref{sec:exp_components}} to confirm its effectiveness in interleaved queries and updates.
\zl{
(Addressing \textcolor{Purple}{\ref{mrw2}, \ref{r1w1}, \ref{r1d8}, \ref{r2w3}, \ref{r2d4}, \ref{r2d7}, \ref{r3d2}})
}

\item \textbf{GPU-CPU-Disk Tires}: We have revised \hl{Section~\ref{sec:overview}} to clarify the GPU-CPU-disk cooperative workflow, expanded \hl{Section~\ref{sec:hierarchical_structure}} to explain the details of this architecture, and \hl{Section~\ref{sec:avc}} to describe the cache replacement algorithm across all three tiers. In \hl{Section~\ref{sec:exp_components}}, we have added experimental validation on the billion-scale dataset.
\zl{
(Addressing \textcolor{Purple}{\ref{mrw7}, \ref{r2w3}, \ref{r2d2}, \ref{r2d6}, \ref{r3w1}})
}

\item \textbf{Dataset and Workloads}: In \hl{Section~\ref{sec:exp_setup}}, we have expanded our evaluation to include mixed query-insertion workloads from Quake~\cite{mohoney2025quake} and two large-scale image datasets (Deep1B~\cite{deep1b}, Text2Image~\cite{text2image}).
\zl{
(Addressing \textcolor{Purple}{\ref{mrw1}, \ref{r1d5}, \ref{r3w3}})
}

\item \textbf{Comparable Baselines}: In \hl{Section~\ref{sec:sanns_performance}} \& \hl{Section~\ref{sec:exp_components}}, we have added GGNN~\cite{GGNN} as an additional baseline to compare the performance under streaming ANNS workloads. We have added LFU and LRFU as baselines to evaluate the efficiency of our caching strategies.  
\zl{
(Addressing \textcolor{Purple}{\ref{mrw5}, \ref{mrw6}, \ref{r1w2}, \ref{r2d5}, \ref{r3w5}, \ref{r3w6}})
}

\item \textbf{Enhanced Readability and Technical Clarity}: The motivation and contributions have been systematically refined, with the technical exposition and experimental analyses reorganized to enhance overall completeness, clarity, and coherence. (Addressing \textcolor{Purple}{\ref{r1w3}, \ref{r2w1}, \ref{r2w3}, \ref{r2d3}})

%mrw4, r1w3, r1d1, r1d2, r1d3, r1d4, r1d7, r2w1, r2w2, r2d3, r2d8,  r2d9, r3w3, r3w4,
\end{enumerate}

We thank the reviewers for their constructive feedback.
% and for the conditional opportunity to revise. 
We propose the following improvements to meet the ``conditional revision'' expectations for the real-time latencies and the interactions between interleaved queries and updates for clearly identified target workloads:
% , we have addressed these issues through three key improvements:
(1) introduced a real-time coordination mechanism with CUDA multi-stream optimization and adaptive resource management to ensure low latency under dynamic workloads (\hl{Section~\ref{sec:coordination}});
(2) implemented a concurrency control protocol between interleaved queries and updates in \hl{Section~\ref{sec:cc_update}}; and
(3) clearly defined target streaming workloads and conducted new experiments in \hl{Section~\ref{sec:exp_components}}
evaluating the effectiveness under mixed query–update conditions.
These revisions ensure correct query–update interactions and demonstrate consistent, low-latency performance across various workloads.

\metareviewersection{}

\begin{metaweakpoint}
\label{mrw1}
The reviews express some skepticism on the real-world needs that require streaming ANN queries. There were also concerns that the access pattern from the MSTuring dataset may not be representative enough. Add more workloads, such as the one in [39] or others, to capture broader dataset characteristics and latency/throughput requirements. Clearly identify the target workload(s), and define what is acceptable latency and throughput for these workloads.
\end{metaweakpoint}

\begin{response}{~\ref{mrw1}}
We thank the reviewers for this valuable feedback. We have substantially revised our paper with real-world use cases, representative access pattern analysis on more workloads, and analyzed the latency and throughput for these workloads to address these concerns.

(1) \textbf{Real-world motivation}: We have added concrete streaming ANNS use cases in \hl{Section~\ref{sec:intro}}, including RAG systems, e-commerce platforms, and video analytics to demonstrate the practical importance of our problem.

(2) \textbf{Broader access pattern analysis}: We have revised \hl{Section~\ref{sec:avc}} (\hl{Figure~\ref{fig:score_analysis}}) to analyze vector access patterns across MSTuring~\cite{msturing} and Tex2image~\cite{text2image} with different dimensions and data types, including images, to demonstrate the generality.

(3) \textbf{Extended workload evaluation}: In \hl{Section~\ref{sec:exp_setup}}, we have expanded our experimental workload with mixed query-insertion workloads following Quake~\cite{mohoney2025quake}, and experiments on Deep1B~\cite{deep1b} and Text2Image datasets to capture broader dataset characteristics.
In \hl{Section~\ref{sec:sanns_performance}}, we have added detailed latency and throughput analysis with clearly defined performance targets (\hl{Figure~\ref{fig:sanns_performance} - Figure~\ref{fig:replacement_comparison}}). 
 
These revisions demonstrate that our approach achieves consistent low-latency performance across realistic real-time workloads. Under varying query–update ratios, SVFusion consistently delivers lower and more stable latency compared with FreshDiskANN and HNSW.

\end{response}

\begin{metaweakpoint}
\label{mrw2}
Present a solution with correct interleaved queries and updates for these target workloads.
\end{metaweakpoint}

\begin{response}{~\ref{mrw2}}
We sincerely thank the reviewers for their incisive feedback.
In this revision, we have incorporated a \textbf{concurrency control} mechanism to ensure correctness for interleaved queries and updates. We have clarified the corresponding techniques in \hl{Section~\ref{sec:cc_update}} and added evaluation under the target workloads in \hl{Section~\ref{sec:exp_components}}.

\textbf{(1) Concurrency Control.} 
We have added \hl{Section~\ref{sec:cc_update}} to present a comprehensive concurrency control protocol that combines fine-grained locks over shared data structures, a two-phase cross-tier synchronization mechanism for atomic visibility, and a multi-version mechanism for snapshot isolation. This mechanism ensures serializability for all interleaved queries and updates across multi-tiers.

\textbf{(2) Experimental Validation.} 
To validate correctness under mixed workloads, we conducted stress tests with interleaved insertions and searches at a 1:1 ratio (\hl{Section~\ref{sec:exp_components}}). As shown in Table~\ref{tab:consistency_ablation}, SVFusion maintains stable Recall@1=0.96 across 500–10K QPS, whereas synchronization-free baselines drop sharply to 0.18. Even at 10K QPS, synchronized operations achieve a p99 latency of 33.2 ms.
These results demonstrate that our concurrency control protocol ensures strong read-after-write consistency and robust low-latency performance under realistic, high-throughput streaming workloads.

% To verify correctness under mixed workloads, we conducted stress tests where insertions and searches are interleaved at a 1:1 ratio (\hl{Section~\ref{sec:exp_components}}). As summarized in Table~\ref{tab:consistency_ablation}, SVFusion maintains stable Recall@1 = 0.96 across 500–10K QPS, while naive synchronization-free baselines degrade sharply (0.18 Recall@1). The p99 latency with synchronization can be finished in 33.2 ms under QPS=10,000.
% These results confirm that our protocol achieves strong read-after-write consistency and robust performance under realistic, high-throughput, and low-latency streaming conditions.
\end{response}

\begin{table}[h]
\centering
\caption*{\changeone{Table 3: Impact of consistency guarantee.}}
\label{tab:consistency_ablation}
\changeone{
\small
\begin{tabular}{l|cccc|cccc}
\toprule
$\backslash$ \textbf{QPS} & \multicolumn{4}{c|}{\textbf{Recall@1}} & \multicolumn{4}{c}{\textbf{p99 Latency (ms)}} \\
& 500 & 2K & 5K & 10K & 500 & 2K & 5K & 10K \\
\midrule
w/ sync  & 0.96 & 0.96 & 0.96 & 0.96 & 4.3  & 6.7 & 10.8 & 33.2\\
w/o sync  & 0.96 & 0.74 & 0.51 & 0.18 & 4.3  & 4.8 & 5.5  & 7.4\\
\bottomrule
\end{tabular}
}
\end{table}

\begin{metaweakpoint}
\label{mrw3}
Experimentally evaluate the query latency of the system. Study the impact of the batch size on latency. Compare the competing methods in terms of latency.
\end{metaweakpoint}

\begin{response}{~\ref{mrw3}}
We thank the reviewers for this valuable suggestion. Guided by these comments (e.g., \rw{r1w1}, \rw{r1w2}, \rw{r2d5}), we have substantially expanded our experimental evaluation to include comprehensive latency analysis. 


(1) We have added \textbf{latency analysis} experiments in \hl{Section~\ref{sec:sanns_performance}} (\hl{Figure~\ref{fig:sanns_lantency}}) where we control the streaming data generation rate (QPS ranging from 500 to 10,000) and measure p50, p95, and p99 latencies for both search and insertion operations across all competing methods. 

(2) We have supplemented our \textbf{caching strategy evaluation} in \hl{Section~\ref{sec:exp_components}} (\hl{Figure~\ref{fig:replacement_comparison}}) with latency metrics to demonstrate the impact of different replacement strategies.

(3) We have added evaluation on a \textbf{billion-scale dataset} under the GPU-CPU-disk framework in \hl{Section~\ref{sec:exp_components}} (\hl{Figure~\ref{fig:disk_analysis3}}) to assess latency-recall trade-offs under extreme-scale settings. 

(4) Finally, we have added experiments in \hl{Section~\ref{sec:exp_paras}} (\hl{Figure~\ref{fig:batchsize_analysis}}) specifically studying \textbf{the impact of batch size} on latency.

\end{response}

\begin{metaweakpoint}
\label{mrw4}
Add throughput experiments for different batch sizes.
\end{metaweakpoint}

\begin{response}{~\ref{mrw4}}
We thank the reviewer for this suggestion. 
We have included parameter sensitivity analysis for batch size in \hl{Section~\ref{sec:exp_paras}}, where we analyzed the impact of varying batch sizes on throughput and recall on the Wikipedia dataset. 
We have also added throughput-latency trade-off experiments across different batch sizes (from 1 to $2^{11}$) as shown in \hl{Figure~\ref{fig:batchsize_analysis}b}, demonstrating how batch size affects both throughput and latency simultaneously.
\end{response}

\begin{metaweakpoint}
\label{mrw5}
Compare with different baselines in addition to LRU, in particular, a frequency-based baseline. LRFU and LFU were suggested as good choices.
\end{metaweakpoint}

\begin{response}{~\ref{mrw5}}
We have added both LFU and LRFU as additional caching baselines to our evaluation. The comparison results are presented in \hl{Section~\ref{sec:exp_components}}, including throughput and latency analysis across different workloads (\hl{Figure~\ref{fig:replacement_comparison}}) and the impact of varying GPU memory ratios (\hl{Figure~\ref{fig:gpu_ratio_comparison}}).
The results demonstrate that SVFusion with WAVP achieves the highest throughput and lowest latency, outperforming SVFusion (w/o WAVP), LRFU, LFU, and LRU by up to 7.2$\times$ in throughput and 5.1$\times$ in latency reduction.

\end{response}

\begin{metaweakpoint}
\label{mrw6}
Add an ablation study to evaluate the effectiveness of workload-aware vector placement.
\end{metaweakpoint}

\begin{response}{\ref{mrw6}}
Thanks for the constructive comments. In \hl{Section~\ref{sec:exp_components}} (``Effectiveness of Adaptive Vector Caching''), we evaluate the effectiveness of our caching strategy. We have clarified that without workload-aware vector placement (WAVP), the system falls back to CPU computation for every GPU cache miss without transferring vectors to the GPU. 
Denoted as \emph{SVFusion w/o WAVP}, we include comparisons with this alternative across varying datasets (\hl{Figure~\ref{fig:replacement_comparison}}) and different GPU memory ratios (\hl{Figure~\ref{fig:gpu_ratio_comparison}}), which effectively serves as an ablation study. Results show that 
compared with \emph{SVFusion w/o WAVP}, our system achieves up to 2.1$\times$ higher throughput and 3.2$\times$ lower latency, demonstrating the effectiveness of our adaptive vector placement mechanism.
\end{response}

\begin{metaweakpoint}
\label{mrw7}
Add details about the SSDs' role in the overall design.
\end{metaweakpoint}

\begin{response}{\ref{mrw7}}
We thank the reviewer for this valuable comment. 
We have revised \hl{Section~\ref{sec:overview}} and \hl{Section~\ref{sec:system_design}} to clarify the role of SSDs in our GPU-CPU-disk hierarchical architecture. Specifically, (1) we have revised \hl{Section~\ref{sec:overview}} to clearly explain our GPU-CPU-disk cooperative workflow; 
(2) We have added a comprehensive explanation in \hl{Section~\ref{sec:hierarchical_structure}} of when and how disk storage is incorporated into the hierarchical design, with a detailed discussion of index building on billion-scale datasets;
(3) We have extended \hl{Section~\ref{sec:avc}} to describe the cache replacement algorithm across all three tiers;
(4) Additionally, we have added experimental validation on the Deep1B dataset in \hl{Section~\ref{sec:exp_components}} (\hl{Figure~\ref{fig:disk_analysis}}) to demonstrate the effectiveness of the disk-extended framework.
\end{response}

\begin{reviewersection}
\label{r1}
\end{reviewersection}

\begin{weakpoint}
\label{r1w1}
The paper totally ignores latency. With a batch size of 10,000 queries as suggested, there is roughly one batch per second for the largest datasets. Thus, users with a single query will wait on average half a second, and in the worst case one second to get their results. There is no discussion of workload assumptions that might suggest how many queries an individual user/application submits per second, or whether queries are dependent on one another, so that query n+1 depends on the output from query n.
\end{weakpoint}

\begin{response}{~\ref{r1w1}}
We thank the reviewer for raising these critical concerns about latency and consistency. 
We fully agree that real-world streaming ANNS systems must also support latency-sensitive scenarios such as online recommendations and interactive search. We have substantially revised the paper to clarify the workload assumptions, extend the concurrency control mechanisms, and enrich the implementation and evaluation to comprehensively address the need for both throughput and latency.


(1) \textbf{Workload Assumption and Characterization}:
We have revised \hl{Section~\ref{sec:intro}} to provide concrete real-world examples of streaming ANNS workloads, including large-scale e-commerce platforms handling millions of concurrent queries and live video analytics systems generating continuous streams of embedding vectors.
In these scenarios, real-time indexing is crucial to ensure search results reflect the most recent state, directly affecting both system responsiveness and user experience.

% We have revised \hl{Section~\ref{sec:intro}} to provide real-world examples of streaming ANNS applications that clarify our workload assumptions with explicit query submission rates (measured in QPS) and query dependencies.
% For example, e-commerce platforms like JD.com process concurrent queries with 500 million daily updates (around 6,000 QPS). Real-time indexing is critical for good experience by making sure the search results reflect the most recent product information at the time of user queries.
\begin{figurecl}[!t]
\centering
\includegraphics[width=0.9\linewidth]{figures/concurrency_control.pdf}
\vspace{-1em}
\caption*{\changeone{Figure 6: Illustrating of the Concurrency Control Workflow.}}
\label{fig:cc_control}
\end{figurecl}

(2) \textbf{Optimization for Low Latency}:
To simultaneously support high-throughput and low-latency workloads, we redesigned SVFusion’s real-time coordination mechanism in \hl{Section~\ref{sec:coordination}} to adapt GPU execution strategies dynamically.
To mitigate batching delays, we introduce a \emph{low-latency processing} scheme that integrates CUDA multi-stream coordination and multi-CTA execution.
Furthermore, an adaptive resource management mechanism is developed to allocate GPU resources under varying workload conditions, thereby improving overall GPU utilization.

(3) \textbf{Concurrency Control}:
We design a two-level concurrency control protocol to enable safe and efficient SANNS operations in \hl{Section~\ref{sec:cc_update}}. 
We first establish \emph{consistency guarantees} through fine-grained locking and synchronized data structures, allowing search operations to access a consistent view even under interleaved queries and updates. 
Building on this foundation, a \emph{multi-version mechanism} decouples expensive background consolidation from serial operations via snapshot isolation, enabling concurrent execution without blocking. \hl{Figure~\ref{fig:cc_control}} shows an example of concurrent insertion and search.

(4) \textbf{Implementation Support for Batch and Streaming Execution}:
We have enhanced the system implementation by incorporating a Kafka-based producer-consumer pipeline (\hl{Section~\ref{sec:exp_setup}}), that seamlessly operates in both batch and streaming modes, similar to Spark Streaming. 
This adaptive scheduler efficiently handles varying workloads by issuing latency-sensitive requests as mini-batches (down to batch size 1) for immediate execution, while aggregating larger tasks to maximize throughput.

(5) \textbf{Experimental evaluation}:
To comprehensively evaluate SVFusion’s latency performance under varying streaming intensities, we scale the request rate from low (QPS=500) to high (QPS=10,000) on the MSTuring dataset.
\hl{Figure~\ref{fig:sanns_lantency}} reports the p50, p95, and p99 latencies for both search and insert operations, demonstrating SVFusion's scalable coordination design that maintains high throughput and consistently low latency.
Additionally, we evaluate latency and throughput with different batch sizes (ranging from 1 to $2^{11}$) in \hl{Figure~\ref{fig:batchsize_analysis}}. The results reveal that SVFusion's flexible batch sizing effectively balances throughput and latency according to workload demands, showcasing its adaptability in diverse streaming scenarios.
Moreover, we validate our concurrency control protocol in \hl{Table~\ref{tab:consistency_ablation}} by conducting a stress test, where each batch contains a 50\% mix of insertions and search queries with batch sizes of 10. These results confirm that SVFusion's fine-grained, multi-tier coordination protocol successfully balances consistency and performance in streaming environments.

Overall, these revisions provide a comprehensive and principled response to this concern, addressing key aspects such as workload assumptions, consistency guarantees, and the effectiveness of SVFusion across both batch and streaming scenarios.
\end{response}

\begin{figurecl}[!t] 
\centering
  \includegraphics[width=1.0\linewidth]{figures/latency_qps_legend.pdf}
 \begin{minipage}[t]{\linewidth}    
    \begin{minipage}[c]{0.015\linewidth}
      \raggedleft
      \rotatebox{90}{\footnotesize\parbox{2cm}{\centering \textbf{QPS=500}}}
    \end{minipage}%
    \hspace{0.1em} 
    \begin{minipage}[c]{0.985\linewidth}
      \includegraphics[width=\linewidth]{figures/latency_qps_500.pdf}
    \end{minipage}
  \end{minipage}

  \begin{minipage}[t]{\linewidth}    
    \begin{minipage}[c]{0.015\linewidth}
      \raggedleft
      \rotatebox{90}{\footnotesize\parbox{2cm}{\centering \textbf{QPS=2000}}}
    \end{minipage}%
    \hspace{0.1em} 
    \begin{minipage}[c]{0.985\linewidth}
      \includegraphics[width=\linewidth]{figures/latency_qps_2000.pdf}
    \end{minipage}
  \end{minipage}

  \begin{minipage}[t]{\linewidth}    
    \begin{minipage}[c]{0.015\linewidth}
      \raggedleft
      \rotatebox{90}{\footnotesize\parbox{2cm}{\centering \textbf{QPS=10000}}}
    \end{minipage}%
    \hspace{0.1em} 
    \begin{minipage}[c]{0.985\linewidth}
      \includegraphics[width=\linewidth]{figures/latency_qps_10000.pdf}
    \end{minipage}
  \end{minipage}

\caption*{\changeone{Figure 8: Comparison of p50, p95 and p99 query latencies.}}
\label{fig:sanns_lantency}
\end{figurecl}

\begin{weakpoint}
\label{r1w2}
While the paper compares with LRU, it does not compare with the other commonly employed least-frequently-used (LFU) heuristic that might actually perform much better here than LRU.
\end{weakpoint}

\begin{response}{~\ref{r1w2}}
Thanks for the constructive comments. 
We have revised both the discussion (\hl{Section~\ref{sec:avc}}) and experiments (\hl{Section~\ref{sec:exp_components}}) to clarify the differences between our caching strategy and LRU/LRFU~\cite{lrfu}. 
\hl{Figure~\ref{fig:replacement_comparison}} \& \hl{Figure~\ref{fig:gpu_ratio_comparison}} demonstrate that SVFusion with WAVP achieves the highest throughput and lowest latency, outperforming SVFusion (w/o WAVP), LRFU, LFU, and LRU by up to 7.2$\times$ in throughput and 5.1$\times$ in latency reduction.
These gains arise because traditional cache policies overlook workload dynamics, causing excessive vector replacements and costly CPU–GPU data transfers.
\end{response}

\begin{figure*}[t] 
\centering
  \includegraphics[width=0.92\textwidth]{figures/exp_replacement_legend.pdf}
  \includegraphics[width=\textwidth]{figures/exp_replacement.pdf}
  \vspace{-2em}
  \caption*{\changeone{Figure 9: Comparison of different replacement strategies on update throughput and miss rate.}}
  \label{fig:replacement_comparison}
\vspace{-1em}
\end{figure*}

\begin{figure*}[t] 
\centering
  \includegraphics[width=0.92\textwidth]{figures/gpu_ratio_analysis_legend.pdf}
  \includegraphics[width=\textwidth]{figures/gpu_ratio_analysis.pdf}
  \vspace{-2em}
  \caption*{\changeone{Figure 10: Impact of different GPU memory ratios on update throughput and miss rate.}}
  \label{fig:gpu_ratio_comparison}
  \vspace{-1.2em}
\end{figure*}

\begin{figurecl}[t] 
\centering
\includegraphics[width=\linewidth]{figures/batch_size_analysis.pdf}
  \vspace{-2em}
  \caption*{\changeone{Figure 17: Impact of varying batch size of updates.}}
  \label{fig:batchsize_analysis}
\end{figurecl}

\begin{weakpoint}
\label{r1w3}
The paper is not self contained. It makes assumptions about the graph that depend on earlier work on which it is based, but are not stated explicitly. (see detailed comments)
\end{weakpoint}

\begin{response}{~\ref{r1w3}}
Thanks for your valuable suggestions. We have substantially enhanced the paper to explicitly state all assumptions that were previously implicit. Specifically:
\begin{itemize}
    \item In \hl{Section~\ref{sec:graph_index}}, we have revised the graph definition to explicitly clarify how directional edges are established.
    \item In the second paragraph of \hl{Section~\ref{sec:graph_index}}, we have expanded the discussion of search workflow, including the strategies of entry point selection during iterative graph traversal. 
    \item We have clearly distinguished between two categories of proximity graphs: k-nearest neighbor graphs (KNNG) with a fixed out-degree and relative neighborhood graphs (RNG) with a variable out-degree in \hl{Section~\ref{sec:graph_index}}. We have also explicitly stated that GPU-based methods predominantly adopt KNNG due to its uniform degree structure, which forms the basis of our index.
\end{itemize}



% PRELIMINARY: add some more detailed graph
% Implementation: cargra (difference)
% Contribution: extension
% RELATED WORK

\end{response}

\begin{detailpoint}
\label{r1d1}
It is not clear why one starts with random elements in Algorithm 1.
\end{detailpoint}
\begin{response}{~\ref{r1d1}}
We thank the reviewer for pointing this out.
We have clarified in \hl{Algorithm~\ref{alg:svfusion}} that the candidate pool is initialized with a small set of randomly selected entry points. 
In graph-based ANNS, entry points can be chosen either randomly~\cite{diskann,CAGRA,ParlayANN} or through specialized initialization strategies~\cite{Iwasaki16,ADSampling}.
Following CAGRA~\cite{CAGRA}, we adopt random initialization for two key reasons: (1) to enhance GPU load balancing by distributing query starting points across the graph and avoiding hotspot contention, and (2) to improve robustness under frequent updates by maintaining structural diversity in search initialization.
We have added concise explanations in \hl{Section~\ref{sec:graph_index}} and \hl{Section~\ref{sec:hierarchical_structure}} to explicitly state this rationale.
\end{response}


\begin{detailpoint}
\label{r1d2}
Shouldn't GetNearest() have $q_i$ as an argument?
\end{detailpoint}

\begin{response}{~\ref{r1d2}}
Thanks for your valuable comments. 
We have updated \hl{Algorithm~\ref{alg:svfusion}} to include $q_i$ as an argument.
\end{response}


\begin{detailpoint}
\label{r1d3}
What determines the direction of an edge in the graph? The discussion suggests that nearby nodes are linked, which would motivate an undirected graph.
\end{detailpoint}
\begin{response}{~\ref{r1d3}}
Thanks for your valuable comments. 
Similar to~\cite{diskann,freshdiskann,CAGRA}, the direction of edges in our graph index is determined by the approximate nearest neighbor selection process: an edge $(v_i, v_j)$ exists when vertex $v_i$ selects $v_j$ as one of its neighbors.

We have clarified this throughout the revised manuscript. 
In the first paragraph of \hl{Section~\ref{sec:graph_index}}, we have explicitly defined edge directionality in the graph structure.
We have further added a detailed discussion in the second graph about the directional properties for both k-nearest neighbor graphs (KNNG~\cite{dong2011}) and relative neighborhood graphs (RNG~\cite{NSG}).

Additionally, beginning of \hl{Section~\ref{sec:insertion}}, we have clearly described the edge establishment process during vector insertion. While the establishment involves bidirectional updates for connectivity, each edge maintains its direction based on which vertex selected the other.
\end{response}

\begin{detailpoint}
\label{r1d4}
Theorem 4.1 is trivial and doesn't deserve the prominence attached to it in the paper.
\end{detailpoint}

\begin{response}{~\ref{r1d4}}
We thank the reviewer for the observation. In this revision, we have removed the theorem and its proof, and integrated its statement directly in \hl{Section~\ref{sec:avc}} for a more concise and cohesive presentation.
\end{response}

\begin{detailpoint}
\label{r1d5}
Reference [39] has appeared at OSDI. The workload generator from that work would be good to include in the evaluation.
\end{detailpoint}

\begin{response}{~\ref{r1d5}}
We thank the reviewer for this insightful comment.
In our revision, we have adopted the \emph{MSTuring-IH} workload from the ODSI paper (previously cited as [39], now updated to~\cite{mohoney2025quake}), which represents a dynamic streaming scenario with tightly interleaved insertions and search operations.
This workload complements our existing evaluation by stressing SVFusion’s ability to sustain query quality under large-scale growth and high update intensity. 
Corresponding results are included in \hl{Section~\ref{sec:exp_setup}}, and we have extended \textbf{the latency analysis and ablation studies} (\hl{Section~\ref{sec:sanns_performance}}, and \hl{Section~\ref{sec:exp_components}}) to cover this workload, demonstrating the robustness and scalability of our system across diverse SANNS scenarios.

\end{response}

\begin{figure*}[t] 
\centering
  \includegraphics[width=0.92\linewidth]{figures/workload_legend.pdf}

  \begin{minipage}[t]{\textwidth}      
    \begin{minipage}[c]{0.035\textwidth}
      \raggedleft
      \rotatebox{90}{\small\parbox{2.5cm}{\centering MSTuring-\\IH}}
    \end{minipage}%
    \hspace{0.6em}%  
    \begin{minipage}[c]{0.95\textwidth}
      \includegraphics[width=\linewidth]{figures/workload6.pdf}
    \end{minipage}
  \end{minipage}
  \vspace{-1em}

  \begin{minipage}[t]{\textwidth}      
    \begin{minipage}[c]{0.035\textwidth}
      \raggedleft
      \rotatebox{90}{\small\parbox{2.5cm}{\centering Text2Image-\\Clustered}}
    \end{minipage}%
    \hspace{0.6em}%  
    \begin{minipage}[c]{0.95\textwidth}
      \includegraphics[width=\linewidth]{figures/workload7.pdf}
    \end{minipage}
  \end{minipage}
  \vspace{-1em}
  
  \caption*{\hl{Figure 7: Comparison of recall, search throughput, insert throughput, and miss rate for MSTuring-IH and Text2Image.}}
  \label{fig:sanns_performance}
\vspace{-1em}
\end{figure*}

\begin{detailpoint}
\label{r1d6}
It is not clear whether the competing methods also batch to the extreme degree of the current paper. If not, they are probably superior according to latency.
\end{detailpoint}

\begin{response}{~\ref{r1d6}}
We thank the reviewer for raising this important point regarding batching strategies and their impact on latency.
In our original experiments, CPU-based baselines such as FreshDiskANN and HNSW are limited by their CPU thread pool size, which constrains the degree of batching they can exploit. In contrast, SVFusion leverages GPU massive parallelism to efficiently process large batches, naturally favoring high-throughput scenarios. 

To address the latency concern and ensure fair evaluation, we have made two key revisions. First, we have added new latency-oriented experiments where the Kafka-based producer sends queries one-by-one (\hl{Figure~\ref{fig:sanns_lantency}} in \hl{Section~\ref{sec:sanns_performance}}), allowing each system to process requests according to its natural execution model and measuring true end-to-end query latency. 
Second, we have added explicit analysis of how batch size affects the latency-throughput trade-off for SVFusion (\hl{Figure~\ref{fig:scalability}} in \hl{Section~\ref{sec:exp_paras}}), demonstrating that our adaptive coordination mechanism can operate efficiently from single-query processing to large-batch.

\end{response}

\begin{detailpoint}
\label{r1d7}
In the worst case, could an adversarial set of deletions disconnect the proximity graph?
\end{detailpoint}

\begin{response}{~\ref{r1d7}}
We appreciate the reviewer’s insightful question.
In SVFusion, adversarial deletions are explicitly mitigated through a combination of structural redundancy and localized repair mechanisms that jointly preserve global connectivity.

First, each node maintains bidirectional neighborhood links, ensuring that insertions create both forward and reverse connections. This symmetric topology prevents node isolation even when multiple hub nodes are removed.
Second, as discussed in \hl{Section~\ref{sec:delete_handling}}, SVFusion employs a topology-aware repair module that continuously monitors degree distribution and local connectivity. Upon detecting structural imbalance, such as loss of bridge edges or degraded neighborhood density, the system proactively reconstructs missing links via localized graph repair, avoiding costly global rebuilds while maintaining reachability across tiers.

We further provide empirical evidence:
\hl{Figure~\ref{fig:delete_distribution}} analyzes deletion patterns under targeted removal of high-degree vertices, confirming that our design effectively captures and repairs critical connectivity losses.
\hl{Figure~\ref{fig:deletion_ablation}} demonstrates that SVFusion sustains a single connected component and stable search accuracy even under adversarial deletion workloads, validating the robustness of our approach against worst-case disconnection scenarios.

% In SVFusion, we address this issue by employing a localized topology-aware repair mechanism in \hl{Section~\ref{sec:delete_handling}}, which continuously detects and rectifies critical connectivity issues in the graph, especially during deletions. This mechanism ensures that even with aggressive or adversarial deletions, the graph remains connected by quickly repairing affected subgraphs before significant fragmentation occurs.

% Moreover, we use incremental sub-graph appending and reverse edge integration to mitigate the effects of deletions on graph connectivity, maintaining structural integrity without the need for expensive global repairs. The design guarantees that the graph is resilient to deletion patterns, preventing the graph from becoming disconnected, even in the worst-case scenarios.


% We have also verified the robustness of this approach through extensive experiments (\hl{Figure~\label{fig:deletion_ablation}} in \hl{Section~\ref{sec:exp_components}}) to ensure that SVFusion consistently maintains graph connectivity, even under extreme deletion patterns.
\end{response}

\begin{detailpoint}
\label{r1d8}
Batching prevents true transactional/serializable behavior when queries are interleaved with updates.
\end{detailpoint}

\begin{response}{\ref{r1d8}}
We thank the reviewer for pointing out the potential limitations of batching on transactional behavior and serializability.

To address this concern, we have implemented a concurrency control protocol in \hl{Section~\ref{sec:cc_update}}, which ensures serializability and consistency across CPU-GPU memory tiers. This protocol leverages fine-grained locking, cross-tier synchronization, and multi-version mechanisms, all of which guarantee safe interleaving of queries and updates, maintaining consistency without sacrificing performance.

Additionally, we have significantly enhanced our design with real-time coordination mechanisms that allow for low-latency processing (\hl{Section~\ref{sec:coordination}}), breaking free from the strict batching model. This enables us to achieve high throughput and low latency simultaneously, adapting dynamically to both batch-oriented and low-latency query requirements.

We have also expanded our evaluation to validate the effectiveness of these mechanisms. As shown in \hl{Table~\ref{tab:consistency_ablation}} (\hl{Section~\ref{sec:exp_components}}), our stress tests reveal that without synchronization, recall degrades drastically (from 0.96 to 0.18), demonstrating the importance of the strong consistency guarantees. With our protocol, however, SVFusion maintains stable recall across varying loads, while introducing acceptable latency overhead, thereby validating its read-after-write consistency.

These revisions emphasize that our system is designed to handle both high-throughput and low-latency workloads without sacrificing transactional integrity, ensuring consistency even when queries and updates are interleaved.
\end{response}

\begin{reviewersection}
\label{r2}
\end{reviewersection}

\begin{weakpoint}
\label{r2w1}
Delta paper.
\end{weakpoint}

\begin{response}{\ref{r2w1}}
We thank the reviewer for prompting us to better clarify our contributions. We have revised \hl{Section~\ref{sec:intro}} to articulate our key novelty: while existing ANNS systems face a fundamental trade-off between dynamic updates and superior performance (higher throughput and lower latency), SVFusion resolves this by enabling concurrent queries and updates across heterogeneous GPU-CPU-disk hierarchies. This poses non-trivial challenges in cross-tier consistency and coordinated processing of different hardware that existing systems do not address.

As in the revised version, our contributions go far beyond incremental improvements, which require fundamental architecture designs. Simply extending existing CPU-based methods~\cite{freshdiskann,hnsw} with GPU acceleration fails due to excessive data transfer overhead, while adapting GPU-based methods~\cite{CAGRA,GGNN,FusionANNS,PilotANN} to support updates breaks their core assumption of static, GPU-resident data. The challenges are fundamental: (1) We need a workload-aware placement strategy that jointly optimizes vector computation and data transfer, going beyond traditional caching that assumes data is always fetched before computation; (2) We must maintain consistency across memory tiers under concurrent operations without sacrificing the parallelism benefits of heterogeneous hardware, a problem existing single-tier systems never face. 
Addressing these challenges requires coordinated co-design of data placement, concurrency control protocols, and workload adaptation across the entire CPU-GPU-disk hierarchy instead of trivial incremental patches.
\end{response}

\begin{weakpoint}
\label{r2w2}
The solution is quite complicated; it is unclear how practical it is.
\end{weakpoint}
\begin{response}{\ref{r2w2}}
We appreciate the reviewer’s concerns regarding the complexity of the solution. We acknowledge that the design of SVFusion is sophisticated; however, this complexity is a direct result of the need to address the challenges inherent in real-world high-dimensional vector search scenarios, particularly for \textbf{large-scale, high-throughput streaming applications}.


To clarify the practical motivation, we emphasize that these challenges are not just theoretical but are faced by industry practitioners working with massive datasets and resource constraints:

(1) \textbf{High-dimensional vectors and large-scale data}: As the size and dimensionality of datasets grow beyond the capacity of traditional systems, especially with GPU memory limitations, novel approaches like ours are critical to efficiently handle massive data volumes. Existing systems like Milvus~\cite{Milvus} and FAISS-GPU~\cite{faiss} highlight the widespread adoption of heterogeneous architectures in industrial applications, where GPU acceleration and memory hierarchies are leveraged to support high-throughput searches. SVFusion builds upon and extends these practices, offering scalable solutions that are essential for real-world workloads.

(2) \textbf{Streaming data with frequent updates}: In dynamic environments where data is continuously updated (e.g., instant search, online product recommendation and live-video monitoring), ensuring consistent indexing and efficient query processing is paramount. Our solution tackles these real-time challenges by dynamically adapting to workload patterns and supporting both batch and streaming queries. This adaptability, while increasing design complexity, is crucial for providing low-latency responses in update-intensive environments.

(3) \textbf{Modularity and Generality}: We have designed SVFusion to be modular, enabling it to integrate with different index structures. This ensures that it can be tailored to diverse application scenarios. 
Evaluation in \hl{Section~\ref{sec:evaluation}} demonstrates its effectiveness across diverse datasets, various workload patterns, and different scales, showcasing its general applicability for both research and industrial streaming ANNS scenarios.

In summary, while SVFusion's design is indeed complex, this complexity is driven by the need to support large-scale and high-throughput streaming applications in a modular manner. The GPU-CPU-disk co-processing design and concurrency control are essential for handling modern streaming workloads and ensuring both high throughput and low latency under heavy updates. 
% Without these sophisticated designs, it would be impossible to meet the demands of emerging real-world use cases, and thus, a more complex solution is both necessary and practical.
\end{response}

\begin{weakpoint}
\label{r2w3}
Some details are missing.
\end{weakpoint}
\begin{response}{\ref{r2w3}}
Thanks for the valuable suggestions. 
We have substantially expanded \hl{Section~\ref{sec:system_design}} \& \hl{Section~\ref{sec:index_update}} to provide comprehensive details. Specifically, we have: (1) detailed our hierarchical index architecture in \hl{Section~\ref{sec:hierarchical_structure}} \& \hl{Section~\ref{sec:avc}}, including how disk is used to store vectors and ANNS; (2) added real-time processing techniques in \hl{Section~\ref{sec:coordination}}, covering low-latency streaming execution, adaptive resource management, and GPU cold-start solutions; (3) introduced a new \hl{Section~\ref{sec:cc_update}} on concurrency control with our two-level protocol for consistency under interleaved queries and updates. 
These details provide the necessary technical depth for understanding and reproducing our system.
\end{response}

\begin{detailpoint}
\label{r2d1}
Motivation and background are relatively compact and well written. Nit: can you provide some real-world examples where streaming ANNs is used, and why this is an important problem.
\end{detailpoint}

\begin{response}{~\ref{r2d1}}
We thank the reviewer for this insightful suggestion. We have expanded the second paragraph of \hl{Section~\ref{sec:intro}} with concrete real-world examples of streaming ANN applications, including RAG systems for emergency response~\cite{streaming_rag}, e-commerce platforms like JD.com~\cite{Vearch}, and live-video analytics for surveillance systems~\cite{rong2021scheduling}. 
In summary, modern systems must maintain fresh indices while achieving high throughput and low latency under continuous updates.
Otherwise, the outdated indices directly impact system correctness, user experience, and operational safety. This clarifies why streaming ANNS has become a critical challenge in production environments.
\end{response}

\begin{detailpoint}
\label{r2d2}
Section 3. When you build a graph that is larger than GPU you partition it. Are you building each partition on GPU and aggregate them on CPU? What if the total graph is bigger than CPU memory?
\end{detailpoint}

\begin{response}{~\ref{r2d2}}
We thank the reviewer for raising this important point regarding index construction under large-scale datasets. 

SVFusion adopts a \textbf{partition-based GPU construction strategy}. For datasets exceeding GPU memory capacity, SVFusion partitions the dataset and constructs each subgraph on the GPU, followed by CPU-side merging to ensure cross-partition connectivity and consistency. For datasets exceeding CPU memory capacity, SVFusion employs a three-tier GPU-CPU-disk architecture, where partitioned subgraphs are built and written to disk, and then merged on CPU within a bounded memory window through on-demand loading.

In the revision, we have clarified the detailed workflow of the index-building process in \hl{Section~\ref{sec:overview}} and \hl{Section~\ref{sec:hierarchical_structure}}, and cache replacement in \hl{Section~\ref{sec:avc}} when the total graph exceeds CPU memory capacity.
Additionally, we have expanded the experimental analysis of the multi-tier framework using the Deep1B dataset~\cite{deep1b} in \hl{Section~\ref{sec:exp_components}}. 
In \hl{Figure~\ref{fig:disk_analysis1} \& Figure~\ref{fig:disk_analysis3}}, we report detailed results on index construction, throughput, and latency. These results demonstrate that SVFusion outperforms DiskANN by achieving over 5$\times$ faster index construction and 2$\times$ higher throughput.
\end{response}

\begin{figurecl}[!t]
    \centering
    \captionsetup[subfigure]{skip=2pt} % 设置子图标题与图片的间距
    \begin{subfigure}[t]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/disk_analysis1.pdf}
        \caption{Construction time}
        \label{fig:disk_analysis1}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[t]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/disk_analysis3.pdf}  
        \caption{Recall-Latency} %  
        \label{fig:disk_analysis3}
    \end{subfigure}
    \hfill%
    \begin{subfigure}[t]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/disk_analysis2.pdf}
        \caption{Recall-Throughput}
        \label{fig:disk_analysis2}
    \end{subfigure}%
    \vspace{-3mm}
    \caption*{\changeone{Figure 11: Effect of GPU-CPU-disk framework}}
    \label{fig:disk_analysis}
\end{figurecl}

\begin{detailpoint}
\label{r2d3}
In general that are a lot of details missing from the high-level description of the four operations. I guess that you will provide details later, so perhaps you can forward reference to the Section containing the details. This will make readers more confident that the details will come later.
\end{detailpoint}

\begin{response}{~\ref{r2d3}}
We thank the reviewer for the constructive suggestion. 
To improve readability and provide a clearer roadmap for the technical details, we have added forward references from \hl{Section~\ref{sec:overview}} to the respective sections describing each operation in depth. 

The revised text now points readers to \hl{\emph{Build} ($\S\ref{sec:hierarchical_structure}$), \emph{Search} (\S\ref{sec:hierarchical_structure} and \S\ref{sec:avc}), \emph{Insertion} (\S\ref{sec:insertion}), and \emph{Deletion} (\S\ref{sec:delete_handling})}.
These cross-references ensure that readers are guided to the detailed algorithmic and system-level discussions that follow, enhancing the coherence between the overview and subsequent sections.

\end{response}

\begin{detailpoint}\label{r2d4}
You are maintaining two copyes of the data between CPU ang GPU (and eventually disk). This will be a problem for deletions, but in Section 4 there is no mention to this. I think it woud be useful to have a callout about the problem here and how you plan to solve it (I guess the details will come later in the paper).
\end{detailpoint}

\begin{response}{~\ref{r2d4}}
We appreciate the reviewer for highlighting the importance of maintaining consistency across multiple memory tiers (GPU, CPU, and disk), particularly during index updates. 
This is indeed a crucial aspect to ensure the correctness and reliability of our system.
To address this concern, we have made three targeted revisions:

(1) At the end of \hl{Section~\ref{sec:hierarchical_structure}}, we now explicitly introduce the cross-tier consistency challenge and outline our design principles, including immediate bitset synchronization and batched structural updates, with a forward reference for further details.

(2) We have added a \textbf{Concurrency Control} subsection in \hl{Section~\ref{sec:cc_update}} to include a dedicated discussion on cross-tier data consistency. This elaborates our two-level synchronization mechanism, which ensures correctness through atomic bitset updates while minimizing transfer overhead.

(3) We evaluate the effectiveness of the concurrency control protocol in \hl{Section~\ref{sec:exp_components}} under an interleaved mix of 50\% insertion and 50\% search queries, and these results in \hl{Table~\ref{tab:consistency_ablation}} demonstrate that our fine-grained, multi-tier coordination protocol effectively balances consistency and performance in high-throughput SANNS scenarios.

\end{response}

\begin{detailpoint}
\label{r2d5}
How different is your caching strategy that LRFU. LRU is quite naive, a comparison against LRFU looks more appropriate (Identifying Hot and Cold Data in Main-Memory Databases, ICDE 2013).
\end{detailpoint}

\begin{response}{~\ref{r2d5}}
We thank the reviewer for this valuable comment and for suggesting a more appropriate baseline. 
We have revised both the discussion (\hl{Section~\ref{sec:avc}}) and experiments (\hl{Section~\ref{sec:exp_components}}) to clarify the differences between our caching strategy and LRFU~\cite{lrfu}.
The evaluated results in \hl{Figure~\ref{fig:replacement_comparison}} demonstrate that \emph{SVFusion with WAVP} achieves the highest throughput and lowest latency, outperforming \emph{SVFusion (w/o WAVP)}, \emph{LRFU}, \emph{LFU}, and \emph{LRU} by up to 7.2$\times$ in throughput and 5.1$\times$ in latency reduction.


% Our approach differs from LRFU in two fundamental aspects:
% (1) \textbf{Caching criterion}. While traditional cache replacement policies, such as LRU and LRFU, are designed to maximize cache hit ratios, our method addresses a broader CPU–GPU co-processing decision, jointly optimizing data transfer overhead and computational efficiency by determining whether to cache a data block on GPU or compute it directly on CPU.
% (2) \textbf{Structural feature space}. Unlike LRFU, which models only temporal locality via recency and frequency, our caching predictor also incorporates graph-structural connectivity, allowing it to identify high-connectivity vectors that act as traversal hubs with higher access likelihood.



\end{response}

\begin{detailpoint}
\label{r2d6}
It is not clear to me how do you warmup the GPU index to avoid startup slowdowns since everything is in CPU.
\end{detailpoint}

\begin{response}{~\ref{r2d6}}
We thank the reviewer for this valuable question. 
To address the concern, we clarify that SVFusion incorporates a dedicated GPU warm-up mechanism to mitigate startup latency and ensure high performance from the first query batch. 
We have added a new paragraph titled \textbf{Cold Start Handling} in \hl{Section~\ref{sec:avc}}, which explains our three-phase initialization process: (1) GPU resource priming to preallocate computation streams and memory pools, (2) data structure setup for index metadata and memory mapping, and (3) cache warm-up guided by our prediction function that prioritizes vectors corresponding to highly connected nodes in the index graph. For datasets exceeding GPU capacity, vectors are ranked and preloaded until the GPU memory is saturated, ensuring immediate responsiveness without startup slowdowns.
\end{response}

\begin{detailpoint}
\label{r2d7}
I feel that there are several details missing in 4.4. Why do you need to partition GPU memory and have spinlocks? Since you are doing batching, what happens if an update comes in while you are doing a search? Are you using MVCC? How do you adapt to the workload? This latter point is not clear at all how do you achieve this and how manual or automatic this is.
\end{detailpoint}

\begin{response}{~\ref{r2d7}}
We thank the reviewer for identifying the insufficient details. 
In this revision, we have explained and clarified our key optimizations regarding performance and concurrency in \hl{Section~\ref{sec:coordination}} and \hl{Section~\ref{sec:cc_update}}:
\begin{itemize}
    \item \textbf{GPU memory Partitioning:} Our system employs multiple concurrent CUDA streams for parallel query processing in \hl{Section~\ref{sec:coordination}}. To mitigate memory contention from these concurrent accesses to shared GPU data structures, we partition GPU memory into independent segments guarded by lightweight spinlocks, with vectors mapped to segments via hashing. 
    \item \textbf{Concurrency Control}: SVFusion employs a \textbf{fine-grained lock-based concurrency control protocol} (\hl{Section~\ref{sec:cc_update}}) rather than MVCC to ensure graph consistency under interleaved updates and searches. 
    In particular, vector search traverses neighbor lists under read locks.
    When insertions occur during search, they acquire read locks for candidate search and write locks only on affected neighbor lists during edge establishment, allowing concurrent searches on unaffected regions to proceed without blocking.
    Deletions update the shared bitset under exclusive lock while marking the affected version, allowing concurrent searches to skip logically deleted vertices without traversal disruption. We have added \hl{Figure~\ref{fig:cc_control}} to illustrate this protocol.
    Additionally, SVFusion employs MVCC specifically for expensive background consolidation, maintaining a small set of consistent graph snapshots across memory tiers to decouple background structural repairs from online operations without blocking.
    The efficiency of this mechanism is validated in \hl{Section~\ref{sec:exp_components}}.
    \item \textbf{Adaptive Resource Management:}  
    SVFusion dynamically allocates GPU resources across concurrent CUDA streams based on their processing overhead, and continuously adjusts the caching threshold $\theta$ based on observed miss rates and the distribution of estimated future access counts $F_\lambda(x)$. (detailed in \hl{Section~\ref{sec:coordination}}). All adaptations operate automatically without manual tuning.
\end{itemize} 
\end{response}

\begin{detailpoint}
\label{r2d8}
The rank-based candidate reordering strategy for insertion is not clear at all.
\end{detailpoint}

\begin{response}{~\ref{r2d8}}
We thank the reviewer for the valuable comment. 
In the revised manuscript, we have substantially rewritten \hl{Section~\ref{sec:insertion}} to provide a precise, formal, and step-by-step explanation of this process.
The core idea of our strategy is to rank candidates based on their structural redundancy (measured by detourable path counts) to prioritize structurally unique connections. This enables efficient neighbor selection while reducing costly distance computations.
\end{response}

\begin{detailpoint}
\label{r2d9}
Please add the PCIe generation you are using in your setup.
\end{detailpoint}

\begin{response}{~\ref{r1d1}}
Thanks for the comment. 
We have added the PCIe generation (PCIE 3.0) in \hl{Section~\ref{sec:exp_setup}}.
\end{response}

\begin{reviewersection}
\label{r3}
\end{reviewersection}

\begin{weakpoint}
\label{r3w1}
The authors mention that SVFusion incorporates disks to store vectors. However, there lacks details about how SSDs are used to store vectors/ in ANNS. In the experiments part, there also lacks experiments to show how disks play their roles in the ANNS search process.
\end{weakpoint}

\begin{response}{~\ref{r3w1}}
We thank the reviewer for raising this important point.
To address this, we have made the following improvements for both technical completeness and experimental validation:
\begin{itemize}
    \item \textbf{GPU–CPU–Disk Cooperative Workflow}. As detailed in \hl{Section~\ref{sec:overview}}, SVFusion adopts a hierarchical storage architecture that seamlessly integrates GPU, CPU, and disk tiers. Vectors are first cached within GPU and CPU memory for fast access, and are subsequently spilled to disk once the host memory capacity is exceeded.
    \item \textbf{Index Construction across Storage Tiers}. In \hl{Section~\ref{sec:hierarchical_structure}}, we have added a comprehensive explanation of when and how disk storage is incorporated into the hierarchical design. The revised text elaborates on the index construction pipeline across GPU, CPU, and disk tiers, including partition-based subgraph building, cross-tier merging, and synchronization to maintain consistency.
    \item \textbf{Cache Replacement and Disk Management}. We further extend the cache replacement algorithm to support disk-level storage upon cache misses in \hl{Section~\ref{sec:avc}}. A lightweight hash-based mapping table is maintained to record vector residency between CPU memory and disk, enabling lookup and migration without introducing significant management overhead.
    \item \textbf{Experimental Validation}. In \hl{Section~\ref{sec:exp_components}}, we introduce new experiments evaluating SVFusion’s performance on billion-scale datasets that exceed CPU memory capacity. The results confirm that the proposed disk-extended framework effectively preserves query efficiency under extreme data volumes shown in \hl{Figure~\ref{fig:disk_analysis}}.
\end{itemize}

\end{response}

\begin{weakpoint}
\label{r3w2}
In Section 4.3, the author shows the vector access patterns on the MSTuring dataset. I wonder whether it is representative enough since its vectors have relatively small dimensions. It would be better if more types of datasets could be included (e.g., images).
\end{weakpoint}

\begin{response}{~\ref{r3w2}}
We thank the reviewer for this valuable suggestion. 
We have revised \hl{Section~\ref{sec:avc}} (\hl{Figure~\ref{fig:score_analysis}}) to include additional analysis of vector access patterns across diverse dataset types. 
Furthermore, we have added two large-scale image datasets to our evaluation: Deep1B~\cite{deep1b} and Text2Image~\cite{text2image}, as detailed in \hl{Section~\ref{sec:exp_setup}} (\hl{Table~\ref{tab:datasets}}). 
Moreover, we have conducted comprehensive SANNS experiments on these image datasets, with results presented in \hl{Figure~\ref{fig:sanns_performance}}.
\end{response}

\begin{figurecl}[t]
    \centering   
    \begin{subfigure}{0.495\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/access_count_analysis.pdf}\
        \vspace{-2em}
        \caption{Distribution of Recent Access.}
        \label{fig:score_analysis_1}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/in_edge_analysis.pdf}\
        \vspace{-2em}
        \caption{Distribution of In-neighbors.}
        \label{fig:score_analysis_2}
    \end{subfigure}
    \vspace{-2em}
    \caption*{\changeone{Figure 4: Characterization of Vector Access Patterns.}}
    \label{fig:score_analysis}
\end{figurecl}

\begin{weakpoint}
\label{r3w3}
This paper proposes a cache manager and a workload-aware vector placement strategy to better utilize buses. However, it is unclear how these components take effect in SVFusion. An ablation study (e.g., performance tests without cache manager/workload-aware vector placement) is needed for these components.
\end{weakpoint}

\begin{response}{~\ref{r3w3}}
We appreciate the reviewer's suggestion. To address this concern, in the evaluation of \textbf{Effectiveness of Adaptive Vector Caching} in \hl{Section~\ref{sec:exp_components}}, we have explicitly defined a baseline named \emph{SVFusion w/o WAVP}, where the workload-aware vector placement is disabled for the ablation study. Using this baseline, the system directly performs distance computation on the CPU without adaptive data transfer decisions upon GPU cache misses. We have conducted comprehensive comparisons between SVFusion and this baseline across multiple workloads (\hl{Figure~\ref{fig:replacement_comparison}}) and under varying GPU memory constraints (\hl{Figure~\ref{fig:gpu_ratio_comparison}}). The results demonstrate that our workload-aware vector placement mechanism contributes significantly to system performance, with SVFusion achieving 2.1$\times$ higher throughput and 3.2$\times$ lower latency compared to \emph{SVFusion w/o WAVP}.
\end{response}

\begin{weakpoint}
\label{r3w4}
The description of the machine may not be correct. A single Xeon Gold 5218 CPU has only 16 CPU cores. As the authors state that the machine has 64 CPU cores, it seems that the machine has 4 CPUs rather than a single CPU. Also, it is better to specify the SSD model and the memory bandwidth of the main memory.
\end{weakpoint}

\begin{response}{~\ref{r3w4}}
We thank the reviewer for this careful observation. 
We have two Intel Xeon Gold 5218 CPUs in our server (forming two NUMA nodes), which provide a total of 32 cores rather than the 64 cores incorrectly stated in the original submission. 
In this revision, we have corrected the hardware configuration in \hl{Section~\ref{sec:exp_setup}} and added the missing hardware specifications as suggested to accurately reflect our experimental setup: the SSD model (\hl{Intel D3-S4510 960 GB enterprise SSDs}) and memory bandwidth (\hl{256 GB/s with 12 channels for DDR4 DRAM}).
\end{response}

\begin{weakpoint}
\label{r3w5}
As the machine has 64 cores with Hyper Threading Technology, it may not be reasonable to use only 16 threads. I think it would be fair to use 32/64/128 threads for testing to fully utilize resources in one or more CPUs.
\end{weakpoint}

\begin{response}{\ref{r3w5}}
We sincerely thank the reviewer for the careful and insightful feedback. 
We have clarified in our evaluation setting that we follow the configuration of the NeurIPS 2023 Big ANN Streaming Challenge~\cite{nips_2023_streaming}. This benchmark uses 16 threads for insertion and 16 threads for search.
To address the reviewer's concern about CPU resource utilization, we have added scalability experiments in \hl{Section~\ref{sec:exp_paras}} (\hl{Figure~\ref{fig:scalability}}) to evaluate how SVFusion and competing methods scale with varying numbers of threads. Note that we vary the number of threads from 1 to 64, as our machine has 32 cores with Hyper Threading Technology (as mentioned in \rw{r3w4}). Results show that all methods exhibit throughput growth as thread count increases. 
Results demonstrate that SVFusion exhibits good scalability with increasing thread counts, confirming the effectiveness of our system design across different CPU resource configurations.
% \textcolor{red}{However, when scaling from 16 to 32 and then to 64 threads, the throughput improvement becomes marginal with an average gain of only 1.24$\times$, suggesting that 16 threads serves as a meaningful experimental configuration, as the relative performance relationships among methods remain consistent even with higher thread counts.
% }
\end{response}

% \begin{figurecl}[t] 
% \centering
%   \includegraphics[width=0.5\linewidth]{figures/detailed_scalability.pdf}
%   \vspace{-1em}
%   \caption*{\hl{Figure 14: Effect of \#Threads.}}
%   \label{fig:scalability}
% \end{figurecl}

\begin{figurecl}[!t]
    \centering

    \begin{minipage}[t]{0.46\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/detailed_scalability.pdf}
        \vspace{-2em}
        \caption*{\hl{Figure 14: Effect of number of threads.}}
        \label{fig:scalability}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gpu_comparison.pdf}
        \vspace{-2em}
        \caption*{\hl{Figure 15: Comparison of GPU-based methods}}
        \label{fig:gpu_comparison}
    \end{minipage}

\end{figurecl}

\begin{weakpoint}
\label{r3w6}
It is not a good idea to use modified FreshDiskANN and HNSW as competitors. The authors’ modifications simply offload distance computation to the GPU, which can easily lead to performance degradation problems due to small memory transfer events, small computation workload, and many synchronization steps. It would be better to choose other competitors for experiments (e.g., GGNN, which uses hierarchical graphs similar to HNSW on GPU).
\end{weakpoint}

\begin{response}{\ref{r3w6}}
We sincerely thank the reviewer for this insightful comment. We have added GGNN~\cite{GGNN} as an additional baseline in our evaluation (\hl{Section~\ref{sec:exp_setup}}). However, GGNN is originally designed for static datasets that fit within GPU memory capacity. To enable fair comparison under dynamic streaming workloads, we extended GGNN to support dynamic update operations through its hierarchical graph structure. For datasets exceeding GPU memory capacity, we implemented a naive fallback mechanism that transfers vectors from CPU to GPU on demand upon cache misses. We evaluated GGNN's performance across various streaming workloads as shown in \hl{Figure~\ref{fig:sanns_performance}}, and compared with other GPU methods in \hl{Figure~\ref{fig:gpu_comparison}}.
\end{response}

\begin{detailpoint}
\label{r3d1}
In the introduction, it is better to specify some scenarios where ANNS on real-time indexes rather than simply citing.
\end{detailpoint}

\begin{response}{~\ref{r3d1}}
We thank the reviewer for this insightful suggestion. 
In the revised manuscript, we have expanded \hl{Section~\ref{sec:intro}} with a more detailed discussion of practical streaming ANN scenarios, including RAG systems, e-commerce platforms, and live-video analytics.   
Please refer to \rw{r1w1}\&\rw{r2d1} for more details of our responses.
\end{response}

\begin{detailpoint}
\label{r3d2}
More discussion about how ANNS and index updating affect each other can be included.
\end{detailpoint}

\begin{response}{~\ref{r3d1}}
We thank the reviewer for this suggestion. We have added a section of \textbf{Concurrency Control} (\hl{Section~\ref{sec:cc_update}}) to address how concurrent ANNS queries and index updates interact in our multi-tier architecture. In this section, we discuss the consistency challenges that arise when queries and updates interleave across CPU-GPU memory tiers, and present our two-level protocol (\hl{Figure~\ref{fig:cc_control}}) that combines fine-grained locking and multi-version snapshots to ensure both correctness and efficiency. 
Moreover, we have added experimental validation in \hl{Table~\ref{tab:consistency_ablation}} to demonstrate that our approach maintains stable recall (0.96) and acceptable latency (33.2 ms) under extreme query-update interleaving across varying loads.
\end{response}

% \bibliographystyle{ACM-Reference-Format}
% \bibliography{coverletter} 

% \end{multicols}

% \twocolumn

\clearpage

% zl: uncomment and use the following commands to mark the changes in the revision paper.
% \changeone{\rone{R1.W2 \\ R1.W3}\textbf{Challenge 3 XXX.}  
% XXX XXX.
% }
